EgoExo-Fitness: Towards Egocentric and Exocentric Full-Body Action Understanding

We present EgoExo-Fitness, a new full-body action understanding dataset, featuring fitness sequence videos recorded from synchronized egocentric and fixed exocentric (third-person) cameras. Compared with existing full-body action understanding datasets, EgoExo-Fitness not only contains videos from first-person perspectives, but also provides rich annotations. Specifically, two-level temporal boundaries are provided to localize single action videos along with sub-steps of each action. More importantly, EgoExo-Fitness introduces innovative annotations for interpretable action judgement--including technical keypoint verification, natural language comments on action execution, and action quality scores. Combining all of these, EgoExo-Fitness provides new resources to study egocentric and exocentric full-body action understanding across dimensions of "what", "when", and "how well". To facilitate research on egocentric and exocentric full-body action understanding, we construct benchmarks on a suite of tasks (i.e., action classification, action localization, cross-view sequence verification, cross-view skill determination, and a newly proposed task of guidance-based execution verification), together with detailed analysis. Code and data will be available at https://github.com/iSEE-Laboratory/EgoExo-Fitness/tree/main.

==> tables/Sequence_list.tex <==
\begin{table}[t]
    \centering
    
    \caption{\textbf{All recorded fitness sequences.} For the correspondence between action names and abbreviations, please refer to \cref{tab:motion_category_appendix}. SID: sequence ID.}
    \vspace{-0.2cm}
    \label{tab:sequence_list}
    \scriptsize
    % \setlength{\extrarowheight}{1pt}%
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{ll|ll} %p{1cm}p{4.25cm}|p{1cm}p{4.25cm}
    \toprule
    \textbf{SIDs} & \textbf{Action Orders} & \textbf{SIDs} & \textbf{Action Orders}\\
    \midrule
    % \,\,1 & KPU, SU, JJ                     &  \,\,30 & KTT, KPU, KRAMC, SU, JJ, HK      & \,\,59 & SB, CJ, KRAMC, HK, SS \\ 
    % \,\,2 & KPU, JJ, SU                     &  \,\,31 & KPU, KTT, KRAMC, SU, JJ, HK  & \,\,60 & SB, CJ, KRAMC, KTT, SS \\ 
    % \,\,3 & KTT, SU, JJ                     &  \,\,32 & KPU, KTT, KRAMC, HK, JJ, SU  & \,\,61 & SB, CJ, KRAMC, LLKL, SS \\
    % \,\,4 & KTT, JJ, SU                     &  \,\,33 & KTT, KRAMC, SU, LLKL, JJ, HK & \,\,62 & SB, CJ, KRAMC, SU, SS \\ 
    % \,\,5 & SU, KTT, JJ                     &  \,\,34 & KTT, JJ, SU, LLKL, KRAMC, HK         & \,\,63 & JJ, SB, KRAMC, CJ, SS \\ 
    % \,\,6 & KPU, JJ, HK                     &  \,\,35 & KRAMC, KTT, SU, LLKL, JJ, HK         & \,\,64 & LLKL, SB, KRAMC, CJ, SS \\
    % \,\,7 & KPU, HK, JJ                     &  \,\,36 & PU, LRL, CJ                          & \,\,65 & PU, SB, LRL, KRAMC, CJ, SS \\
    % \,\,8 & JJ, KPU, HK                     &  \,\,37 & LRL, PU, CJ                          & \,\,66 & PU, SB, LRL, CJ, SS, KRAMC \\
    % \,\,9 & KPU, SU, LLKL, JJ               &  \,\,38 & SB, CJ, LRL                          & \,\,67 & PU, LRL, SB, KRAMC, CJ, SS \\
    % \,\,10 & KPU, SU, JJ, LLKL              &  \,\,39 & LRL, SB, CJ                          & \,\,68 & SB, PU, SU, LRL, CJ, SS \\
    % \,\,11 & SU, KPU, LLKL, JJ              &  \,\,40 & PU, LRL, KRAMC, CJ                   & \,\,69 & SB, PU, LLKL, LRL, CJ, SS \\
    % \,\,12 & KTT, SU, LLKL, JJ              &  \,\,41 & PU, LRL, CJ, KRAMC                   & \,\,70 & PU, SB, SU, SS, CJ, LRL \\
    % \,\,13 & KTT, SU, JJ, LLKL              &  \,\,42 & LRL, PU, KRAMC, CJ                   & \,\,71 & PU, SB, JJ, SS, CJ, LRL \\
    % \,\,14 & LLKL, SU, KTT, JJ              &  \,\,43 & SB, LRL, KRAMC, CJ           & \,\,72 & PU, SB, LLKL, SS, CJ, LRL \\
    % \,\,15 & KPU, KTT, JJ, HK               &  \,\,44 & SB, LRL, CJ, KRAMC \         & \,\,73 & PU, SB, KTT, SS, CJ, LRL \\
    % \,\,16 & KPU, KTT, HK, JJ               &  \,\,45 & KRAMC, LRL, SB, CJ           & \,\,74 & SB, HK, LRL, KRAMC, CJ, SS \\
    % \,\,17 & KTT, KPU, JJ, HK               &  \,\,46 & PU, SB, CJ, SS               & \,\,75 & SB, CJ, LRL, KRAMC, JJ, SS \\
    % \,\,18 & KPU, KTT, SU, LLKL, JJ         &  \,\,47 & PU, SB, SS, CJ               & \,\,76 & SU, SB, LRL, KRAMC, CJ, SS\\
    % \,\,19 & KPU, KTT, SU, JJ, LLKL         &  \,\,48 & SB, PU, CJ, SS               & \,\,77 & LLKL,KRAMC,HK \\
    % \,\,20 & KPU, SU, KTT, LLKL, JJ         &  \,\,49 & PU, SB, LRL, KRAMC, CJ       & \,\,78 & SB,LRL,CJ \\
    % \,\,21 & KTT, KPU, SU, JJ, HK           &  \,\,50 & PU, SB, LRL, CJ, KRAMC       & \,\,79 & PU,SB,CJ,LRL \\
    % \,\,22 & KPU, KTT, SU, JJ, HK           &  \,\,51 & PU, LRL, SB, KRAMC, CJ       & \,\,80 & KTT,SU,JJ,HK \\
    % \,\,23 & KPU, KTT, HK, JJ, SU           &  \,\,52 & SB, PU, LRL, CJ, SS          & \,\,81 & KPU,KTT,SU,JJ \\
    % \,\,24 & KTT, KRAMC, LLKL, JJ, HK       &  \,\,53 & PU, SB, LRL, CJ, SS          & \,\,82 & KPU,KTT,LLKL,SU,JJ,HK \\
    % \,\,25 & KTT, JJ, LLKL, KRAMC, HK       &  \,\,54 & PU, SB, SS, CJ, LRL          & \,\,83 & KPU,KTT,JJ,HK,LLKL \\
    % \,\,26 & KRAMC, KTT, LLKL, JJ, HK       &  \,\,55 & SB, HK, KRAMC, CJ, SS        & \,\,84 & PU,SB,KRAMC,CJ,SS \\
    % \,\,27 & KPU, KTT, SU, LLKL, JJ, HK     &  \,\,56 & SB, KTT, KRAMC, CJ, SS       & \,\,85 & KPU,SU,KTT,KRAMC,JJ \\
    % \,\,28 & KPU, KTT, SU, JJ, HK, LLKL     &  \,\,57 & SB, KPU, KRAMC, CJ, SS       & \,\,86 & KTT,KRAMC,LLKL,SU,JJ,HK \\
    % \,\,29 & KPU, SU, KTT, LLKL, JJ, HK     &  \,\,58 & SB, CJ, KRAMC, KPU, SS \\
    \,\,1 & KPU, SU, JJ                     &  \,\,44 & SB, LRL, CJ, KRAMC     \\ 
    \,\,2 & KPU, JJ, SU                     &  \,\,45 & KRAMC, LRL, SB, CJ     \\ 
    \,\,3 & KTT, SU, JJ                     &  \,\,46 & PU, SB, CJ, SS         \\ 
    \,\,4 & KTT, JJ, SU                     &  \,\,47 & PU, SB, SS, CJ         \\ 
    \,\,5 & SU, KTT, JJ                     &  \,\,48 & SB, PU, CJ, SS         \\          
    \,\,6 & KPU, JJ, HK                     &  \,\,49 & PU, SB, LRL, KRAMC, CJ \\          
    \,\,7 & KPU, HK, JJ                     &  \,\,50 & PU, SB, LRL, CJ, KRAMC \\          
    \,\,8 & JJ, KPU, HK                     &  \,\,51 & PU, LRL, SB, KRAMC, CJ \\          
    \,\,9 & KPU, SU, LLKL, JJ               &  \,\,52 & SB, PU, LRL, CJ, SS    \\          
    \,\,10 & KPU, SU, JJ, LLKL              &  \,\,53 & PU, SB, LRL, CJ, SS    \\          
    \,\,11 & SU, KPU, LLKL, JJ              &  \,\,54 & PU, SB, SS, CJ, LRL    \\          
    \,\,12 & KTT, SU, LLKL, JJ              &  \,\,55 & SB, HK, KRAMC, CJ, SS  \\          
    \,\,13 & KTT, SU, JJ, LLKL              &  \,\,56 & SB, KTT, KRAMC, CJ, SS \\          
    \,\,14 & LLKL, SU, KTT, JJ              &  \,\,57 & SB, KPU, KRAMC, CJ, SS \\          
    \,\,15 & KPU, KTT, JJ, HK               &  \,\,58 & SB, CJ, KRAMC, KPU, SS \\          
    \,\,16 & KPU, KTT, HK, JJ               &  \,\,59 & SB, CJ, KRAMC, HK, SS \\        
    \,\,17 & KTT, KPU, JJ, HK               &  \,\,60 & SB, CJ, KRAMC, KTT, SS \\       
    \,\,18 & KPU, KTT, SU, LLKL, JJ         &  \,\,61 & SB, CJ, KRAMC, LLKL, SS \\      
    \,\,19 & KPU, KTT, SU, JJ, LLKL         &  \,\,62 & SB, CJ, KRAMC, SU, SS \\        
    \,\,20 & KPU, SU, KTT, LLKL, JJ         &  \,\,63 & JJ, SB, KRAMC, CJ, SS \\        
    \,\,21 & KTT, KPU, SU, JJ, HK           &  \,\,64 & LLKL, SB, KRAMC, CJ, SS \\      
    \,\,22 & KPU, KTT, SU, JJ, HK           &  \,\,65 & PU, SB, LRL, KRAMC, CJ, SS \\   
    \,\,23 & KPU, KTT, HK, JJ, SU           &  \,\,66 & PU, SB, LRL, CJ, SS, KRAMC \\   
    \,\,24 & KTT, KRAMC, LLKL, JJ, HK       &  \,\,67 & PU, LRL, SB, KRAMC, CJ, SS \\   
    \,\,25 & KTT, JJ, LLKL, KRAMC, HK       &  \,\,68 & SB, PU, SU, LRL, CJ, SS \\      
    \,\,26 & KRAMC, KTT, LLKL, JJ, HK       &  \,\,69 & SB, PU, LLKL, LRL, CJ, SS \\    
    \,\,27 & KPU, KTT, SU, LLKL, JJ, HK     &  \,\,70 & PU, SB, SU, SS, CJ, LRL \\      
    \,\,28 & KPU, KTT, SU, JJ, HK, LLKL     &  \,\,71 & PU, SB, JJ, SS, CJ, LRL \\      
    \,\,29 & KPU, SU, KTT, LLKL, JJ, HK     &  \,\,72 & PU, SB, LLKL, SS, CJ, LRL \\
    \,\,30 & KTT, KPU, KRAMC, SU, JJ, HK    &  \,\,73 & PU, SB, KTT, SS, CJ, LRL \\
    \,\,31 & KPU, KTT, KRAMC, SU, JJ, HK    &  \,\,74 & SB, HK, LRL, KRAMC, CJ, SS \\
    \,\,32 & KPU, KTT, KRAMC, HK, JJ, SU    &  \,\,75 & SB, CJ, LRL, KRAMC, JJ, SS \\
    \,\,33 & KTT, KRAMC, SU, LLKL, JJ, HK   &  \,\,76 & SU, SB, LRL, KRAMC, CJ, SS\\
    \,\,34 & KTT, JJ, SU, LLKL, KRAMC, HK   &  \,\,77 & LLKL,KRAMC,HK \\
    \,\,35 & KRAMC, KTT, SU, LLKL, JJ, HK   &  \,\,78 & SB,LRL,CJ \\
    \,\,36 & PU, LRL, CJ                    &  \,\,79 & PU,SB,CJ,LRL \\
    \,\,37 & LRL, PU, CJ                    &  \,\,80 & KTT,SU,JJ,HK \\
    \,\,38 & SB, CJ, LRL                    &  \,\,81 & KPU,KTT,SU,JJ \\
    \,\,39 & LRL, SB, CJ                    &  \,\,82 & KPU,KTT,LLKL,SU,JJ,HK \\
    \,\,40 & PU, LRL, KRAMC, CJ             &  \,\,83 & KPU,KTT,JJ,HK,LLKL \\
    \,\,41 & PU, LRL, CJ, KRAMC             &  \,\,84 & PU,SB,KRAMC,CJ,SS \\
    \,\,42 & LRL, PU, KRAMC, CJ             &  \,\,85 & KPU,SU,KTT,KRAMC,JJ \\
    \,\,43 & SB, LRL, KRAMC, CJ             &  \,\,86 & KTT,KRAMC,LLKL,SU,JJ,HK \\
    \bottomrule
    \end{tabular}
    }
\end{table}
\vspace{-1.5cm}

